SciHorizon-DataEVA: An Agentic System for AI-Readiness Evaluation of Heterogeneous Scientific Data

AI-for-Science (AI4Science) is increasingly transforming scientific discovery by embedding machine learning models into prediction, simulation, and hypothesis generation workflows across domains. However, the effectiveness of these models is fundamentally constrained by the AI-readiness of scientific data, for which no scalable and systematic evaluation mechanism currently exists. In this work, we propose SciHorizon-DataEVA, a novel agentic system to scalable AI-readiness evaluation of heterogeneous scientific data. At the evaluation-criteria level, we introduce the Sci-TQA2 principles, which organize AI-readiness into four complementary dimensions: Governance Trustworthiness, Data Quality, AI Compatibility, and Scientific Adaptability. Each dimension is decomposed into measurable atomic elements that enable fine-grained and executable assessment. To operationalize these principles at scale, we develop Sci-TQA2-Eval, a hierarchical multi-agent evaluation approach orchestrated through a directed, cyclic workflow. Our Sci-TQA2-Eval dynamically constructs dataset-aware evaluation specifications by combining lightweight dataset profiling, applicability-aware metric activation, and knowledge-augmented planning grounded in domain constraints and dataset-paper signals. These specifications are executed through an adaptive, tool-centric evaluation mechanism with built-in verification and self-correction, enabling scalable and reliable assessment across heterogeneous scientific data. Extensive experiments on scientific datasets spanning multiple domains demonstrate the effectiveness and generality of SciHorizon-DataEVA for principled AI-readiness evaluation.

==> 3_Methodology.tex <==
\section{Methodology}

\subsection{Problem Formulation}
In this work, we address the challenge of automating the AI-readiness evaluation for heterogeneous scientific datasets. We formally define the key components and the evaluation objective as follows.

\subsubsection{Preliminaries}
Let $\mathcal{D}$ denote a raw scientific dataset, which typically consists of a set of data files $\{d_1, d_2, \dots, d_n\}$ (e.g., tabular files, images, or molecular graphs) and associated metadata $\mathcal{M}$ (e.g., variable descriptions, licensing info). Unlike general-domain datasets, a scientific dataset is intrinsically bound to a specific scientific domain context $\mathcal{C}$ (e.g., \textit{Computational Fluid Dynamics} or \textit{Genomics}), which dictates the physical laws and constraints the data must obey.

We define the \textbf{AI-Readiness Assessment} as a hierarchical mapping process. For a given tuple $(\mathcal{D}, \mathcal{M}, \mathcal{C})$, the goal is to derive a comprehensive evaluation result $\mathcal{E}$, consisting of a quantitative score vector $\mathbf{s}$ and a qualitative report $\mathcal{R}$.

\textbf{Definition 1 (Hierarchical Evaluation Dimensions).} We construct the evaluation space $\mathcal{S}$ based on four orthogonal dimensions:
\begin{equation}
    \mathcal{S} = \{ \text{Qual}, \text{Gov}, \text{AI}, \text{Sci} \}
\end{equation}
where:
\begin{itemize}
    \item $\text{Qual}$ denotes \textit{Data Quality} (e.g., completeness, noise level).
    \item $\text{Gov}$ denotes \textit{Governance \& Trustworthiness} (e.g., FAIRness, privacy).
    \item $\text{AI}$ denotes \textit{AI Compatibility} (e.g., feature relevance, class balance).
    \item $\text{Sci}$ denotes \textit{Scientific Adaptability} (e.g., physical consistency, boundary coverage).
\end{itemize}
The final score vector is represented as $\mathbf{s} \in [0, 1]^4$, where each component $s_k$ corresponds to the normalized score of dimension $k \in \mathcal{S}$.

% To provide an intuitive metric for human experts, we further define the \textbf{Overall AI-Readiness Score} $S_{total} \in [0, 100]$ as the scaled mean of the dimension vector:
% \begin{equation}
%     S_{total} = 100 \times \frac{1}{4} \sum_{i \in \{\text{qual, gov, ai, sci}\}} s_i
%     \label{eq:total_score}
% \end{equation}
% Thus, the final output of our system is a tuple $(\mathbf{s}, S_{total}, \mathcal{R})$, containing the fine-grained vector, the overall score, and the diagnostic report.

\subsubsection{Task Definition}
Conventionally, data evaluation is modeled as a static function $f_{static}: (\mathcal{D}, \mathcal{M}) \rightarrow \mathbf{s}$, implemented via pre-defined rules (e.g., checking null values). However, in scientific domains, the evaluation logic is highly dependent on the context $\mathcal{C}$. For instance, an outlier in a sensor reading might be a "sensor error" (low quality) or a "rare physical event" (high scientific value), depending on $\mathcal{C}$. Thus, a static $f$ fails to capture the semantic validity of scientific data.

We reformulate the task as a \textbf{Dynamic Tool Generation and Execution} problem. Instead of applying a fixed set of rules, the system must autonomously generate a domain-specific executable tool $\mathcal{T}_{\mathcal{C}}$ (i.e., Python code) to evaluate the dataset.

\textbf{Problem 1 (Agentic AI-Readiness Evaluation).} Given a dataset $\mathcal{D}$, metadata $\mathcal{M}$, and domain context $\mathcal{C}$, the objective is to learn a policy $\pi_{\theta}$ (parameterized by an LLM) that generates a sequence of actions $a_1, \dots, a_T$ to:
\begin{enumerate}
    \item Retrieve domain-specific evaluation standards $\mathcal{K}_{\mathcal{C}}$ from external knowledge bases;
    \item Synthesize an executable evaluation tool $\mathcal{T}_{\mathcal{C}} = \text{Gen}(\mathcal{K}_{\mathcal{C}}, \mathcal{M})$;
    \item Execute $\mathcal{T}_{\mathcal{C}}$ on $\mathcal{D}$ to compute the score vector $\mathbf{s}$ and generate the diagnostic report $\mathcal{R}$.
\end{enumerate}
Formally, we seek to maximize the reliability and validity of the generated assessment:
\begin{equation}
    \mathcal{T}_{\mathcal{C}}^* = \arg\max_{\mathcal{T}} \mathbb{E} \left[ \text{Validity}(\mathcal{T}(\mathcal{D}) \mid \mathcal{C}) \right]
\end{equation}
where $\text{Validity}(\cdot)$ measures how well the evaluation reflects the true utility of the data for downstream scientific AI tasks.
% where $\text{Validity}(\cdot)$ measures the quality of the generated tool. In our framework, this validity is composed of two constraints: (1) \textit{Executability} (the tool runs without errors), and (2) \textit{Semantic Alignment} (the evaluation logic aligns with scientific domain consensus). This objective function directly motivates our self-correction mechanism described in Sec. 3.4.

\subsection{The Hierarchical Evaluation System}
The proposed evaluation system adopts a hierarchical structure to provide a comprehensive assessment of a dataset's AI-readiness. This system is organized into four primary dimensions, as shown in Figure 1.
Unlike traditional frameworks that focus solely on intrinsic data properties, our system explicitly incorporates the requirements of modern AI modeling and the rigor of scientific discovery:

\begin{itemize}
    \item \textbf{Data Quality:} Evaluates the technical purity and standardization of the data, ensuring it can be processed by algorithms with minimal manual cleaning. 
    \item \textbf{Governance Trustworthiness:} Focuses on the long-term reusability and safety of the data within legal and ethical frameworks. It ensures that the data collection and sharing processes are compliant and transparent. 
    \item \textbf{AI Compatibility:} Measures the technical utility of the data for machine learning, examining whether the dataset contains sufficient signals for various model architectures and effective training. 
    \item \textbf{Scientific Adaptability:} Addresses the depth and breadth of the data in the context of scientific research, ensuring it supports genuine discovery rather than mere statistical fitting. It gauges the data's ability to represent underlying physical laws and diverse experimental regimes.
\end{itemize}

To achieve a more granular assessment, each sub-dimension is further refined into \textbf{atomic evaluation elements}. While several of these elements are domain-agnostic, others are highly dependent on domain knowledge for meaningful instantiation and quantification. This adaptation process allows the framework to align its evaluative criteria with the specific requirements of different scientific disciplines. For example, while the evaluation of \textit{Data Scale} in a general context might rely on absolute sample counts, its scientific assessment must be calibrated against the inherent rarity of specific phenomena, such as protein structures or rare astronomical events. Similarly, evaluating the \textit{Operating Conditions Coverage} requires domain-specific insights into physical parameter spaces, such as identifying whether data samples span across critical phase transition points or stay within narrow, linear regimes. This mechanism ensures that the evaluation is both mathematically rigorous and scientifically relevant. A detailed definition of all hierarchical dimensions, sub-dimensions, and their corresponding atomic elements is provided in the Appendix.

Based on this multi-dimensional evaluation, we can generate a comprehensive assessment report designed to guide both data optimization and downstream research applications. The report provides a quantitative breakdown of the dataset's performance across the defined dimensions, offering a diagnostic analysis of its strengths and limitations. Based on Data Quality and Governance dimensions, we can deliver clear directions for dataset improvement, such as identifying required cleaning steps, standardizing units, or highlighting missing licensing information. Furthermore, the Scientific Adaptability dimension enables the report to assess the potential for scientific discovery, identifying whether the data is sufficient for causal inference or if it lacks coverage in critical physical regimes necessary for robust generalization. This analysis is paired with the AI Compatibility dimension to recommend suitable AI model architectures and learning strategies, such as suggesting graph neural networks for molecular datasets or few-shot learning techniques for high-scarcity data. Ultimately, the report serves as a bridge between data curators and AI researchers, facilitating more informed decisions in the AI for Science workflow.

% \begin{table*}[t]
% \centering
% \caption{The Hierarchical Evaluation Taxonomy of Sci-DARE. The system covers four core dimensions, extending from basic quality to scientific utility.}
% \label{tab:evaluation_taxonomy}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l|l}
% \toprule
% \textbf{Dimension} & \textbf{Sub-Dimension} & \textbf{Core Objective / Definition} \\
% \midrule
% \multirow{5}{*}{\textbf{D1. Data Quality}} 
%  & Completeness & Absence of missing values and structural integrity of records. \\
%  & Accuracy & Reflection of objective physical reality; absence of measurement errors. \\
%  & Uniqueness & Absence of duplicate records or redundant samples. \\
%  & Consistency & Uniformity of formats, units, and encoding standards. \\
%  & Timeliness & Alignment with current scientific knowledge and experimental states. \\
% \midrule
% \multirow{5}{*}{\textbf{D2. Governance}} 
%  & FAIRness & Adherence to Findable, Accessible, Interoperable, and Reusable principles. \\
%  & Provenance \& Licensing & Clarity of ownership, usage rights (e.g., CC licenses), and lineage. \\
%  & Privacy & Protection of sensitive information (e.g., PII in medical data). \\
%  & Bias & Absence of selection bias in population, geography, or instrumentation. \\
%  & Scientific Ethics & Compliance with ethical norms (e.g., animal welfare, dual-use risks). \\
% \midrule
% \multirow{6}{*}{\textbf{D3. AI Compatibility}} 
%  & AI Model Adaptability & Suitability for diverse AI architectures (e.g., CNNs, GNNs, Neural Operators). \\
%  & Data Scale & Absolute scale regarding sample size, feature dimensionality, and storage. \\
%  & Class Balance & Uniformity of sample distribution across different categories or outcomes. \\
%  & Class Separability & Distinction in feature space; theoretical difficulty of the classification task. \\
%  & Feature Importance & Strength of correlation between features and target variables (Signal vs. Noise). \\
%  & Data Point Value & Information density contained within individual samples. \\
% \midrule
% \multirow{4}{*}{\textbf{D4. Sci. Adaptability}} 
%  & Task Generalizability & Ability to support multiple downstream scientific tasks, not just a single proxy. \\
%  & Data Scarcity & The difficulty of acquisition, reproducibility, and uniqueness of the data. \\
%  & Causal Completeness & Inclusion of sufficient variables (confounders) to infer causal relationships. \\
%  & Condition Coverage & Breadth of coverage across physical parameter spaces (e.g., temperature, pressure). \\
% \bottomrule
% \end{tabular}%
% }
% \end{table*}

\subsection{The Agentic Framework Architecture}

The implementation of Sci-DARE is grounded in a hierarchical multi-agent system (MAS) orchestrated via a directed cyclic graph (DCG) workflow. Unlike static pipelines, our architecture decouples \textit{semantic reasoning} from \textit{code execution}, enabling the system to dynamically adapt to the heterogeneity of scientific data. The framework comprises four collaborative modules: Semantic Perception, Strategy Planning, Evolvable Tool Engine, and Reporting.

\subsubsection{Semantic Perception and Task Grounding}
The foundation of our framework lies in correctly interpreting the raw data environment and mapping it to the appropriate scientific context. This module consists of the \texttt{Data Inspector}, the \texttt{Knowledge Base}, and the \texttt{Evaluator}.

\paragraph{Data Inspector.}
This component acts as the sensory front-end. It scans the target directory to extract the \textbf{Data Profile} ($\mathcal{P}_{data}$), which encapsulates the file tree structure, detected file formats (e.g., \texttt{.csv}, \texttt{.pdb}, \texttt{.nc}), and accessible metadata headers. The inspector infers the data modality (e.g., tabular, graph, sequence) and basic statistics without loading the full payload, ensuring efficiency on petabyte-scale scientific datasets.

\paragraph{Knowledge Base (KB) Construction.}
The KB serves as the semantic anchor for domain adaptation. We construct it through a rigorous, two-pronged approach:
\begin{itemize}
    \item \textbf{Domain-Specific Element Knowledge (Type-I):} To support fine-grained evaluation elements, we build a semi-structured database for each scientific domain. For every (Domain, Element) tuple, we pre-define a knowledge schema containing specific fields required for assessment. The content for these fields is extracted from a vast corpus of domain-specific literature, ensuring the evaluation criteria align with the latest scientific consensus.
    \item \textbf{Dataset-Paper Pairs (Type-II):} To provide task-aware insights, we construct a relational graph linking datasets to downstream AI applications. We first extract dataset mentions from massive scientific literature and then cross-reference them with open-science repositories (e.g., Papers With Code, Hugging Face, Zenodo). This results in a comprehensive \textit{Dataset-Paper Pairs} database, allowing the system to infer a dataset's "AI Compatibility" and "Scientific Adaptability" by analyzing how similar data has been utilized in existing AI-for-Science research.
\end{itemize}

\paragraph{Evaluator.}
Acting as a semantic filter, the \texttt{Evaluator} bridges the \textit{Data Profile} and the hierarchical taxonomy defined in Sec 3.2. It queries the Type-I knowledge in the KB to determine the \textit{Applicability} of each evaluation element. For instance, if the Inspector detects a multi-file directory with image-text pairs, the Evaluator activates the \texttt{ModalAlignment} element; otherwise, it prunes this branch. The output is a tailored \textit{Evaluation Manifest}, listing only the relevant elements to be processed.

\subsubsection{Collaborative Strategy Planning}
The \texttt{Planner} agent functions as the cognitive core ("The Brain"). Upon receiving the Evaluation Manifest, it executes a dual-stage reasoning process to transform abstract goals into executable blueprints.

\paragraph{Stage I: Data-Load Strategy.}
Scientific data often exceeds memory limits or requires specialized parsing. The Planner first formulates a loading strategy ($\pi_{load}$) based on the file structure in $\mathcal{P}_{data}$ and the requirements of the active evaluation elements. 
\begin{itemize}
    \item \textit{Targeting}: Deciding whether to load the full dataset, specific columns (e.g., "only coordinates $x,y,z$"), or metadata headers.
    \item \textit{Sampling}: For massive datasets, the Planner defines a sampling policy (e.g., "random sampling" for distribution checks vs. "time-slice sampling" for temporal consistency).
\end{itemize}

\paragraph{Stage II: Evaluation Strategy.}
Once data is accessible, the Planner formulates the quantification strategy ($\pi_{eval}$). By synthesizing the generic definition of a Fine-grained Element with the domain knowledge retrieved from the KB, the Planner re-defines the metric for the specific context.
For example, for the \texttt{Consistency} element in a Climate dataset, the Planner translates the generic "unit check" into a specific instruction: "Verify if the Temperature variable aligns with Kelvin units as defined in the CMIP6 standard found in KB."

\paragraph{Strategy-Level Refinement.}
The Planner maintains a feedback loop with the execution layer. Unlike syntactic errors handled by the Tool Engine, \textit{semantic failures} (e.g., tool execution returns \texttt{None} or logically impossible values like negative mass) trigger a \textbf{Strategic Reflection}. The Planner analyzes whether the failure stems from an incorrect loading strategy (e.g., wrong file parsing) or a misaligned evaluation definition, and iteratively refines the plan $\pi$ before requesting a new tool.

\subsubsection{The Evolvable Tool Engine}
The execution layer of Sci-DARE is designed not merely as a static runtime, but as an evolvable engine capable of "learning" from its interactions with diverse scientific data. This module integrates the \textit{Tool Library}, \textit{Tool Memory}, and the \textit{Code-Making Pipeline} into a self-evolving loop, capable of retrieving, generating, and validating executable tools on the fly.

\paragraph{Structured Tool Library.}
The core asset of the engine is the Tool Library $\mathcal{L}$, which serves as a repository of verified, reusable evaluation logic. To ensure robust manageability without exposing implementation details, we design each tool entry $t \in \mathcal{L}$ as a comprehensive metadata tuple containing:
\begin{itemize}
    \item \textbf{Identity \& Scope}: A unique identifier and the specific \textit{Fine-grained Element}
    \item \textbf{Operational Constraints}: Explicit definitions of accepted \textit{Input Parameters} (e.g., data types like \texttt{pandas.DataFrame} or file paths) and \textit{Domain Applicability} (specifying whether the tool is generic, multi-domain, or strictly domain-specific).
    \item \textbf{Semantic Description}: A natural language summary of the underlying evaluation algorithm and the domain knowledge leveraged during its construction.
    \item \textbf{Encapsulated Implementation}: The executable Python code itself, stored as a self-contained functional unit (including all necessary dependency imports) to ensure atomic execution.
\end{itemize}

\paragraph{Hierarchical Retrieval Mechanism.}
To efficiently locate the optimal tool for a given Planner strategy, we employ a coarse-to-fine retrieval strategy:
\begin{enumerate}
    \item \textit{Hard Filtering}: The engine first subsets $\mathcal{L}$ by matching the target evaluation element and validating that the tool's input parameter types are compatible with the loaded data format.
    \item \textit{Semantic Selection}: The filtered candidates (represented by their IDs, domain scopes, and descriptions) are presented to the LLM agent. Guided by the Planner's specific evaluation method, the agent semantically reasons to select the single most appropriate tool ID.
\end{enumerate}

\paragraph{Tool Memory.}
The engine's reliability is augmented by a distinct \textit{Tool Memory} $\mathcal{M}_{tool}$, which records interaction trajectories to guide future actions. We categorize these memories into three streams:
\begin{itemize}
    \item \textit{Data Loading Logs}: Historical records of successful data parsing strategies, providing references for the \textit{Data Inspector} when encountering similar file structures in the future.
    \item \textit{Success Trajectories}: Logs of successful invocations, serving as few-shot exemplars to inform the Planner on how to correctly parameterize specific tools for specific data types.
    \item \textit{Failure Trajectories}: Records of runtime errors or semantic misalignments. These act as "negative constraints" during the generation of new tools, preventing the recurrence of known pitfalls.
\end{itemize}

\paragraph{Generation and Self-Correction Loop.}
When a "cold start" occurs (no tool found), the engine enters a generative closed-loop involving three specialized roles:
\begin{enumerate}
    \item \textbf{Tool Creator (Architect)}: It synthesizes a coding blueprint based on the Planner's strategy, the loaded data profile, and domain knowledge. This blueprint specifies input interfaces, necessary dependencies (e.g., \texttt{rdkit} for chemistry), and quantitative thresholds.
    \item \textbf{Tool Verification (Reviewer)}: The generated code is executed in a sandboxed environment. The Reviewer acts as a dual-layer critic:
    \begin{itemize}
        \item \textit{Runtime Feedback}: It captures standard errors and triggers a code-level regeneration.
        \item \textit{Semantic Feedback}: It checks if the return value is logically valid (e.g., score $\in [0,1]$). If the output is null or physically impossible, it triggers a strategy-level reflection to the Planner.
    \end{itemize}
    \item \textbf{Update}: Upon successful verification, the new tool is indexed into $\mathcal{L}$, enabling the system to handle similar future tasks without regeneration.
\end{enumerate}

\subsubsection{Experience Consolidation and Reporting}
The final phase synthesizes the fragmented evaluation results into a cohesive scientific report.

\paragraph{Aggregator.}
The \texttt{Aggregator} collects the quantified outputs from all executed tools, normalizing them into the four-dimensional score vector $\mathbf{s}$. It applies a dynamic weighting scheme where the importance of each dimension is adjusted based on the domain context (e.g., "Privacy" is up-weighted for Clinical data).

\paragraph{Insight Generation.}
Beyond numerical scoring, Sci-DARE leverages the \textit{Dataset-Paper Pairs} in the Knowledge Base to mine the \textbf{Latent Potential} of the data. the system traverses the relational graph, analyzing how similar datasets have been repurposed in cutting-edge research. For instance, if Dataset $A$ is structurally similar to Dataset $B$, and Dataset $B$ was successfully used in Paper $P$ for a specific task (e.g., "Protein Folding"), the system infers that Dataset $A$ holds potential for similar applications. 
This process generates an \textbf{AI-Ready Report} that not only diagnoses deficits but also explicitly recommends potential downstream AI tasks and correlate low scores with specific constraints found in successful papers, offering optimation steps.

==> 3_Preliminaries.tex <==


\section{Problem Definition}
Scientific datasets exhibit \emph{heterogeneity} across multiple perspectives, including modality \textcolor{red}{(e.g., tabular measurements, microscopy images, molecular graphs)}, storage organization (single file vs.\ multi-file directory), and \textcolor{red}{representation schemas—the conventions that specify how observations are encoded and interpreted (e.g., standardized variable definitions, unit systems, and annotation protocols). More fundamentally, unlike general-domain datasets whose quality is often assessed via generic statistical regularities, scientific data are inseparable from a \emph{domain context} $C$ (e.g., earth science and materials chemistry). The context $C$ determines the relevant scientific constraints and measurement conventions that the data must satisfy. Consequently, an effective evaluation framework must accommodate the intrinsic heterogeneity of scientific data and the domain-specific semantics imposed by the context $C$, while remaining scalable across datasets, modalities, and scientific disciplines.}


%Scientific datasets exhibit \emph{heterogeneity} along multiple axes, including modality (e.g., tabular measurements, microscopy images, molecular graphs), storage organization (single file vs.\ multi-file directory), and schema (variable naming, units, coordinate systems, and annotation protocols). 
%More fundamentally, unlike general-domain datasets whose validity is often judged by generic statistical regularities, a scientific dataset is intrinsically bound to a \emph{domain context} $C$ (e.g., Computational Fluid Dynamics, Climate Science, Genomics). 
%The context $C$ dictates the governing physical/biological constraints and measurement conventions that the data must obey (e.g., unit systems, conservation laws, admissible ranges, and standardized variable definitions). 
%Consequently, an evaluation framework must account for both surface-level data properties and context-dependent semantic validity.

\begin{definition}[\textbf{Heterogeneous Scientific Dataset Evaluation}] 
Given a raw scientific dataset represented as a set of data files
$D=\{d_1,d_2,\ldots,d_n\}$ (e.g., tables, images, graphs) and associated metadata $M$ (e.g., variable descriptions, provenance, licensing, collection protocol), the goal is to produce a comprehensive evaluation result
$E=(\mathbf{s}, R)$, where $\mathbf{s}\in \mathbb{R}^k$ is a vector of quantitative scores and $R$ is a qualitative diagnostic report 
%\textcolor{red}{containing evidence, failure modes, and actionable recommendations.}
containing evidence and actionable recommendations.
We emphasize that $k$ is not fixed a priori at this stage: $\mathbf{s}$ may include multiple scoring components, each defined according to downstream evaluation principles introduced in subsequent sections.% whose semantics are defined by the downstream evaluation principles.% (introduced in subsequent sections).
\end{definition}


% A key requirement in scientific settings is \emph{domain adaptability}: the evaluation logic must be conditioned on the domain context $C$. This stands in contrast to conventional static evaluation pipelines
% $f_{\text{static}}:(D,M)\rightarrow \mathbf{s}$,
% implemented via predefined generic rules (e.g., missing-value rates, schema checks, or format validation). While such rules are necessary, they are insufficient for scientific datasets because they do not capture whether the data obeys domain-specific semantics (e.g., physically consistent units, valid coordinate conventions, or biologically plausible ranges). Hence, the central challenge is to design an evaluator that is both \emph{computable} on raw data and \emph{semantically grounded} in $C$.

% \begin{definition}[\textbf{Dynamic Tool Generation and Execution.}] 
% To enable domain-adaptive evaluation under heterogeneous data formats, we reformulate the task as a \emph{Dynamic Tool Generation and Execution} problem. Given $(D,M,C)$, the objective is to learn a policy $\pi_\theta$ (parameterized by a large language model) that produces a sequence of actions $\{a_t\}_{t=1}^T$ to:
% \begin{enumerate}
%     \item retrieve domain-specific evaluation standards and constraints $\mathcal{K}_C$ from external knowledge sources;
%     \item synthesize an executable evaluation tool $T_C = \textsc{Gen}(\mathcal{K}_C, M)$ that operationalizes the evaluation logic under context $C$;
%     \item execute $T_C$ on $D$ to compute the score vector $\mathbf{s}$ and generate a diagnostic report $R$.
% \end{enumerate}

% We formalize the goal as maximizing the reliability and context-validity of the assessment produced by the generated tool:
% \begin{equation}
% T_C^{*} = \arg\max_{T \in \mathcal{T}} \ \mathbb{E}\big[ \mathrm{Validity}\big(T(D), C\big) \big]
% \label{eq:tool_opt}
% \end{equation}
% where $\mathcal{T}$ denotes the space of executable tools representable by the system, and $\mathrm{Validity}(\cdot)$ measures whether the produced assessment faithfully reflects the dataset's true utility and trustworthiness for downstream scientific AI tasks under domain context $C$ (e.g., whether the tool detects physically impossible values, inconsistent unit conventions, or domain-specific schema violations that would invalidate model training or benchmarking).
% \end{definition}

% In summary, the evaluation problem studied in this work is not merely to compute generic quality statistics, but to construct and execute context-aware tools that bridge raw heterogeneous data to domain-grounded, actionable assessments.


==> tables/leaderboard_asto_bio.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}
\caption{Quantitative Evaluation Results. Background intensity correlates with score magnitude. 
\textbf{$T$}: Governance Trustworthiness ($T_1$: FAIRness, $T_2$: Provenance, $T_3$: Ethics); \textbf{$Q$}: Data Quality ($Q_1$: Complete., $Q_2$: Acc., $Q_3$: Unique., $Q_4$: Consist.); \textbf{$A^c$}: AI Compatibility ($A^c_1$: Adapt., $A^c_2$: Scale, $A^c_3$: Bal., $A^c_4$: Feat.Imp.); \textbf{$A^s$}: Scientific Adaptability ($A^s_1$: Task Gen., $A^s_2$: Scarcity, $A^s_3$: Causal, $A^s_4$: Cond. Cov.).
\textit{Modality}: \faGlobe~Tensor, \faProjectDiagram~Graph, \faTable~Table, \faImage~Image, \faFont~Text.}
\label{tab:leaderboard_main}

\begin{tabular}{l c c | ccc | cccc | cccc | cccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & 
\multirow{2}{*}{\textbf{Mod.}} & 
\multirow{2}{*}{\textbf{Total}} & 
\multicolumn{3}{c|}{\textbf{Governance ($T$)}} & 
\multicolumn{4}{c|}{\textbf{Quality ($Q$)}} & 
\multicolumn{4}{c|}{\textbf{AI Comp. ($A^c$)}} & 
\multicolumn{4}{c}{\textbf{Sci. Adapt. ($A^s$)}} \\

\cmidrule(lr){4-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18}

 &  &  & $T_1$ & $T_2$ & $T_3$ & $Q_1$ & $Q_2$ & $Q_3$ & $Q_4$ & $A^c_1$ & $A^c_2$ & $A^c_3$ & $A^c_4$ & $A^s_1$ & $A^s_2$ & $A^s_3$ & $A^s_4$ \\
\midrule
\rowcolor{blue!8} \multicolumn{18}{c}{\textit{\textbf{Astronomy}}} \\
\midrule
Ring\_Moat\_Dome\_Str. & \faImage & 88.6 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 99.8 & \gMid 67.5 & \gHigh 100.0 & \gMid 73.4 & \gLow 45.7 & \gHigh 93.8 & \gHigh 93.3 & \gGood 89.0 & \gGood 87.0 \\
Ionospheric\_Obs. & \faGlobe & 88.1 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 86.8 & \gGood 82.4 & \gMid 74.3 & \gHigh 100.0 & \gGood 82.8 & \gGood 78.8 & - & \gBad 0.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 87.6 & \gGood 87.4 \\
Martian\_Aeol.\_Land. & \faImage & 86.2 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 75.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 93.7 & \gHigh 100.0 & \gMid 61.3 & - & \gGood 87.5 & \gGood 86.0 & \gLow 45.3 & \gGood 78.0 \\
SOLAR\_WIND\_MODEL & \faTable & 83.7 & \gGood 80.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 98.0 & \gHigh 90.9 & \gHigh 99.9 & \gHigh 100.0 & \gGood 87.5 & \gHigh 99.3 & \gGood 82.0 & \gBad 15.4 & \gHigh 100.0 & \gHigh 97.0 & \gHigh 93.7 & \gBad 24.2 \\
Solar\_Act.\_AI\_Fore. & \faImage,\faTable & 81.8 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 93.5 & \gGood 88.5 & \gBad 0.0 & \gHigh 100.0 & \gMid 73.3 & \gHigh 100.0 & \gGood 83.4 & \gBad 0.0 & \gHigh 100.0 & \gHigh 94.5 & \gMid 61.3 & \gLow 46.7 \\
Optical\_Star\_Image & \faImage & 81.3 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 98.8 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 92.5 & \gMid 51.8 & \gLow 25.7 & - & \gGood 88.5 & \gMid 58.9 & \gGood 75.0 & \gGood 85.2 \\
LAMOST\_DR5 & \faTable & 80.9 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 81.4 & \gLow 34.4 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 99.1 & \gMid 67.6 & \gMid 52.7 & \gGood 81.0 & \gGood 81.2 & \gHigh 98.0 & \gLow 30.0 & \gMid 57.9 \\
CPk & \faTable & 79.7 & \gGood 80.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gBad 0.0 & \gBad 0.0 & \gHigh 100.0 & \gGood 80.0 & \gHigh 91.8 & \gMid 74.9 & \gLow 40.5 & \gMid 70.0 & \gMid 72.5 & \gMid 51.7 & \gBad 21.2 \\
Solar\_WL\_Flares & \faImage,\faTable,\faGlobe & 78.3 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gLow 46.5 & \gHigh 100.0 & \gGood 75.5 & \gMid 62.1 & \gHigh 100.0 & \gGood 86.8 & - & \gHigh 100.0 & \gHigh 98.3 & \gLow 40.2 & \gMid 50.0 \\
Solar\_Chrom.\_H$\alpha$ & \faImage,\faGlobe & 78.2 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 99.8 & \gHigh 100.0 & \gGood 77.6 & \gMid 73.1 & \gLow 31.9 & - & - & \gGood 82.7 & \gHigh 94.0 & \gLow 40.3 & \gGood 78.5 \\

\rowcolor{green!8} \multicolumn{18}{c}{\textit{\textbf{Biology}}} \\
\midrule
Flysta3D & \faImage & 91.4 & - & - & - & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 99.6 & \gMid 71.2 & - & \gHigh 100.0 & \gHigh 98.1 & \gHigh 100.0 & \gMid 53.3 & - \\
The-Gonzo-Dataset & \faGlobe,\faTable & 86.8 & \gHigh 100.0 & \gMid 55.6 & \gGood 83.3 & \gHigh 100.0 & \gLow 48.8 & - & \gHigh 100.0 & \gHigh 100.0 & \gGood 78.3 & - & - & \gHigh 100.0 & \gHigh 100.0 & \gGood 82.7 & \gHigh 100.0 \\
Synth.-Skeletal-Mot. & \faImage,\faTable & 81.4 & \gHigh 100.0 & \gLow 44.4 & \gGood 83.3 & \gHigh 100.0 & \gMid 50.0 & \gHigh 96.8 & \gHigh 100.0 & \gGood 87.7 & \gMid 68.0 & \gGood 84.5 & \gHigh 91.0 & \gHigh 92.2 & \gMid 60.0 & \gGood 86.3 & \gGood 87.1 \\
MedMNISTv2 & \faGlobe & 80.2 & \gHigh 100.0 & \gMid 55.6 & \gGood 83.3 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 92.1 & \gHigh 100.0 & \gMid 70.0 & \gGood 75.6 & \gGood 80.3 & - & \gGood 85.0 & \gMid 74.7 & \gBad 6.0 & \gGood 85.2 \\
FIVES & \faImage & 80.0 & \gLow 36.0 & \gMid 55.6 & \gMid 58.3 & \gHigh 100.0 & \gBad 0.0 & \gHigh 97.6 & \gHigh 99.4 & \gHigh 90.0 & \gHigh 91.4 & \gHigh 99.8 & - & \gGood 87.5 & \gHigh 92.0 & \gMid 55.0 & \gHigh 96.5 \\
Genomic-benchmarks & \faFont & 79.9 & \gMid 60.0 & \gMid 66.7 & \gMid 66.7 & \gHigh 90.6 & \gGood 78.1 & \gMid 70.0 & \gHigh 100.0 & \gHigh 94.0 & \gGood 79.9 & \gHigh 98.6 & - & \gMid 62.5 & \gGood 80.0 & \gBad 0.0 & \gHigh 96.1 \\
RNA-seq-human-kidney & \faTable & 79.8 & \gMid 60.0 & \gMid 66.7 & \gMid 62.5 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 95.3 & \gMid 64.1 & \gHigh 100.0 & \gBad 0.0 & \gMid 51.2 & \gHigh 100.0 & \gMid 50.7 & - \\
HQColon\_sampled & \faImage,\faGlobe,\faTable & 77.9 & \gMid 56.0 & \gMid 66.7 & \gMid 70.8 & \gBad 0.0 & \gGood 80.6 & \gBad 0.0 & \gGood 87.5 & \gHigh 98.0 & \gGood 81.1 & \gGood 80.4 & - & \gHigh 100.0 & \gHigh 100.0 & \gGood 76.7 & \gBad 16.7 \\
Insect-Odorant-Bind. & \faProjectDiagram,\faTable & 76.8 & \gHigh 96.0 & \gBad 22.2 & \gGood 79.2 & \gGood 87.5 & \gMid 63.5 & \gHigh 99.5 & \gHigh 94.7 & \gHigh 95.5 & \gMid 64.8 & \gHigh 93.7 & \gLow 25.7 & \gHigh 95.5 & \gGood 86.5 & \gGood 75.0 & \gGood 84.9 \\
RAS-Dataset & \faGlobe & 74.8 & \gHigh 96.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 75.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 78.0 & \gGood 86.9 & \gMid 62.5 & \gBad 5.9 & - & \gGood 77.1 & \gHigh 90.0 & \gBad 10.0 & \gMid 64.6 \\

\bottomrule
\end{tabular}
\end{table*}

==> tables/leaderboard_bio_mat.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}
\caption{Quantitative Evaluation Results. Background intensity correlates with score magnitude. 
\textbf{$T$}: Governance Trustworthiness ($T_1$: FAIRness, $T_2$: Provenance, $T_3$: Ethics); \textbf{$Q$}: Data Quality ($Q_1$: Complete., $Q_2$: Acc., $Q_3$: Unique., $Q_4$: Consist.); \textbf{$A^c$}: AI Compatibility ($A^c_1$: Adapt., $A^c_2$: Scale, $A^c_3$: Bal., $A^c_4$: Feat.Imp.); \textbf{$A^s$}: Scientific Adaptability ($A^s_1$: Task Gen., $A^s_2$: Scarcity, $A^s_3$: Causal, $A^s_4$: Cond. Cov.).
\textit{Modality}: \faGlobe~Tensor, \faProjectDiagram~Graph, \faTable~Table, \faImage~Image, \faFont~Text.}
\label{tab:leaderboard_main_bio_materials_chemistry}

\begin{tabular}{l c c | ccc | cccc | cccc | cccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & 
\multirow{2}{*}{\textbf{Mod.}} & 
\multirow{2}{*}{\textbf{Total}} & 
\multicolumn{3}{c|}{\textbf{Gov. Trust. ($T$)}} & 
\multicolumn{4}{c|}{\textbf{Data Qual. ($Q$)}} & 
\multicolumn{4}{c|}{\textbf{AI Comp. ($A^c$)}} & 
\multicolumn{4}{c}{\textbf{Sci. Adapt. ($A^s$)}} \\

\cmidrule(lr){4-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18}

 &  &  & $T_1$ & $T_2$ & $T_3$ & $Q_1$ & $Q_2$ & $Q_3$ & $Q_4$ & $A^c_1$ & $A^c_2$ & $A^c_3$ & $A^c_4$ & $A^s_1$ & $A^s_2$ & $A^s_3$ & $A^s_4$ \\
\midrule
\rowcolor{green!8} \multicolumn{18}{c}{\textit{\textbf{Biology}}} \\
\midrule
Flysta3D & \faImage & 91.4 & \gGood 85.7 & \gHigh 100.0 & \gGood 79.2 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 99.6 & \gMid 71.2 & - & \gHigh 100.0 & \gHigh 98.1 & \gHigh 100.0 & \gMid 53.3 & - \\
The-Gonzo-Dataset & \faGlobe,\faTable & 86.8 & \gHigh 100.0 & \gMid 55.6 & \gGood 83.3 & \gHigh 100.0 & \gLow 48.8 & - & \gHigh 100.0 & \gHigh 100.0 & \gGood 78.3 & - & - & \gHigh 100.0 & \gHigh 100.0 & \gGood 82.7 & \gHigh 100.0 \\
Synth.-Skeletal-Mot. & \faImage,\faTable & 81.4 & \gHigh 100.0 & \gLow 44.4 & \gGood 83.3 & \gHigh 100.0 & \gMid 50.0 & \gHigh 96.8 & \gHigh 100.0 & \gGood 87.7 & \gMid 68.0 & \gGood 84.5 & \gHigh 91.0 & \gHigh 92.2 & \gMid 60.0 & \gGood 86.3 & \gGood 87.1 \\
MedMNISTv2 & \faGlobe & 80.2 & \gHigh 100.0 & \gMid 55.6 & \gGood 83.3 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 92.1 & \gHigh 100.0 & \gMid 70.0 & \gGood 75.6 & \gGood 80.3 & - & \gGood 85.0 & \gMid 74.7 & \gBad 6.0 & \gGood 85.2 \\
FIVES & \faImage & 80.0 & \gLow 36.0 & \gMid 55.6 & \gMid 58.3 & \gHigh 100.0 & \gBad 0.0 & \gHigh 97.6 & \gHigh 99.4 & \gHigh 90.0 & \gHigh 91.4 & \gHigh 99.8 & - & \gGood 87.5 & \gHigh 92.0 & \gMid 55.0 & \gHigh 96.5 \\
Genomic-benchmarks & \faFont & 79.9 & \gMid 60.0 & \gMid 66.7 & \gMid 66.7 & \gHigh 90.6 & \gGood 78.1 & \gMid 70.0 & \gHigh 100.0 & \gHigh 94.0 & \gGood 79.9 & \gHigh 98.6 & - & \gMid 62.5 & \gGood 80.0 & \gBad 0.0 & \gHigh 96.1 \\
RNA-seq-human-kidney & \faTable & 79.8 & \gMid 60.0 & \gMid 66.7 & \gMid 62.5 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 95.3 & \gMid 64.1 & \gHigh 100.0 & \gBad 0.0 & \gMid 51.2 & \gHigh 100.0 & \gMid 50.7 & - \\
HQColon\_sampled & \faImage,\faGlobe,\faTable & 77.9 & \gMid 56.0 & \gMid 66.7 & \gMid 70.8 & \gBad 0.0 & \gGood 80.6 & \gBad 0.0 & \gGood 87.5 & \gHigh 98.0 & \gGood 81.1 & \gGood 80.4 & - & \gHigh 100.0 & \gHigh 100.0 & \gGood 76.7 & \gBad 16.7 \\
Insect-Odorant-Bind. & \faProjectDiagram,\faTable & 76.8 & \gHigh 96.0 & \gBad 22.2 & \gGood 79.2 & \gGood 87.5 & \gMid 63.5 & \gHigh 99.5 & \gHigh 94.7 & \gHigh 95.5 & \gMid 64.8 & \gHigh 93.7 & \gLow 25.7 & \gHigh 95.5 & \gGood 86.5 & \gGood 75.0 & \gGood 84.9 \\
RAS-Dataset & \faGlobe & 74.8 & \gHigh 96.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 75.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 78.0 & \gGood 86.9 & \gMid 62.5 & \gBad 5.9 & - & \gGood 77.1 & \gHigh 90.0 & \gBad 10.0 & \gMid 64.6 \\

\rowcolor{orange!8} \multicolumn{18}{c}{\textit{\textbf{Materials \& Chemistry}}} \\
\midrule
FreeSolv & \faTable,\faProjectDiagram & 88.2 & \gGood 85.7 & \gHigh 100.0 & \gGood79.2 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 99.8 & \gHigh 100.0 & \gMid 56.2 & \gGood 76.2 & \gHigh 96.8 & \gGood 87.5 & \gHigh 97.5 & \gHigh 100.0 & \gHigh 90.3 \\
BigSolDBv2.0 & \faTable & 88.0 & \gHigh 100.0 & \gMid 55.6 & \gGood 83.3 & \gHigh 99.3 & \gHigh 91.3 & \gHigh 100.0 & \gHigh 100.0 & \gGood 89.2 & \gHigh 100.0 & \gGood 80.1 & \gGood 77.6 & \gMid 68.8 & \gHigh 100.0 & \gHigh 95.0 & \gGood 87.5 \\
AIMD & \faProjectDiagram & 87.7 & \gGood 76.0 & \gHigh 100.0 & \gHigh 95.8 & - & - & \gMid 64.6 & \gHigh 97.9 & \gHigh 95.0 & \gMid 72.2 & - & - & \gHigh 93.8 & \gHigh 97.5 & \gHigh 90.0 & \gHigh 100.0 \\
xxMD & \faProjectDiagram & 86.3 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 99.3 & \gHigh 100.0 & \gBad 0.0 & \gHigh 90.6 & \gGood 84.0 & \gMid 71.8 & \gLow 47.6 & \gHigh 100.0 & \gHigh 100.0 & \gLow 48.2 & \gGood 85.4 \\
Raw\_Hyperspec.\_Refl. & \faTable & 85.0 & \gHigh 96.0 & \gHigh 100.0 & \gHigh 95.8 & \gHigh 99.8 & \gHigh 99.4 & \gHigh 100.0 & \gHigh 100.0 & \gGood 81.2 & \gBad 16.0 & \gGood 87.2 & \gMid 73.7 & \gMid 71.2 & \gHigh 100.0 & \gMid 66.7 & \gGood 81.9 \\
1018\_Compounds & \faTable & 85.0 & \gHigh 96.0 & \gHigh 100.0 & \gHigh 95.8 & \gHigh 100.0 & \gMid 71.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 99.9 & \gMid 68.1 & \gHigh 99.4 & - & \gMid 62.5 & \gHigh 90.0 & \gLow 40.0 & \gMid 72.0 \\
TAA.csv & \faTable & 84.5 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 99.0 & \gHigh 100.0 & \gHigh 95.5 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gLow 49.7 & \gLow 30.2 & \gHigh 90.0 & \gBad 0.0 & \gBad 3.4 & \gHigh 96.8 \\
CO2\_Electrocat.\_Red. & \faTable & 81.9 & \gHigh 96.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 98.8 & \gHigh 97.5 & \gHigh 100.0 & \gHigh 97.3 & \gHigh 100.0 & \gGood 88.1 & \gLow 38.7 & - & \gMid 68.4 & \gGood 81.6 & \gMid 57.8 & \gGood 75.0 \\
ML-Driven\_Elast.\_Pred. & \faTable & 78.7 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 91.8 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 98.0 & \gGood 87.5 & \gMid 70.0 & \gMid 55.3 & \gMid 62.5 & \gMid 50.4 & \gLow 44.0 & \gLow 40.2 \\
Hydrogen\_Combustion & \faGlobe & 73.2 & \gLow 36.0 & \gMid 55.6 & \gMid 54.2 & \gHigh 100.0 & - & \gHigh 90.0 & \gHigh 100.0 & \gGood 80.5 & \gHigh 100.0 & \gBad 2.0 & - & \gHigh 96.7 & \gHigh 93.0 & \gMid 67.0 & \gGood 89.4 \\

\bottomrule
\end{tabular}
\end{table*}

==> tables/leaderboard_phy_bio.tex <==
\begin{table*}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{5pt}
\caption{Quantitative Evaluation Results. Background intensity correlates with score magnitude. 
\textbf{$T$}: Governance Trustworthiness ($T_1$: FAIRness, $T_2$: Provenance, $T_3$: Ethics); \textbf{$Q$}: Data Quality ($Q_1$: Complete., $Q_2$: Acc., $Q_3$: Unique., $Q_4$: Consist.); \textbf{$A^c$}: AI Compatibility ($A^c_1$: Adapt., $A^c_2$: Scale, $A^c_3$: Bal., $A^c_4$: Feat.Imp.); \textbf{$A^s$}: Scientific Adaptability ($A^s_1$: Task Gen., $A^s_2$: Scarcity, $A^s_3$: Causal, $A^s_4$: Cond. Cov.).
\textit{Modality}: \faGlobe~Tensor, \faProjectDiagram~Graph, \faTable~Table, \faImage~Image, \faFont~Text.}
\label{tab:leaderboard_main_physics_bio}

\begin{tabular}{l c c | ccc | cccc | cccc | cccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & 
\multirow{2}{*}{\textbf{Mod.}} & 
\multirow{2}{*}{\textbf{Total}} & 
\multicolumn{3}{c|}{\textbf{Governance ($T$)}} & 
\multicolumn{4}{c|}{\textbf{Quality ($Q$)}} & 
\multicolumn{4}{c|}{\textbf{AI Comp. ($A^c$)}} & 
\multicolumn{4}{c}{\textbf{Sci. Adapt. ($A^s$)}} \\

\cmidrule(lr){4-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18}

 &  &  & $T_1$ & $T_2$ & $T_3$ & $Q_1$ & $Q_2$ & $Q_3$ & $Q_4$ & $A^c_1$ & $A^c_2$ & $A^c_3$ & $A^c_4$ & $A^s_1$ & $A^s_2$ & $A^s_3$ & $A^s_4$ \\
\midrule
\rowcolor{red!8} \multicolumn{18}{c}{\textit{\textbf{Physics}}} \\
\midrule
Multiharm.\_Feedback & \faTable & 93.2 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 83.9 & - & \gGood 82.4 & \gMid 66.7 & \gGood 85.0 & \gGood 85.3 & \gHigh 100.0 \\
CdS\_Nanowire\_SHG & \faTable & 88.9 & \gHigh 92.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gMid 55.6 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 96.0 & \gLow 49.4 & - & \gGood 86.6 & \gGood 87.5 & \gHigh 90.0 & \gHigh 90.0 & \gHigh 100.0 \\
Dusty\_Plasma\_Ratchet & \faTable & 86.8 & \gHigh 96.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & - & \gHigh 100.0 & \gHigh 92.9 & \gGood 86.2 & \gMid 70.3 & \gMid 55.5 & \gHigh 94.5 & \gHigh 93.8 & \gLow 25.0 & \gGood 82.9 & \gGood 76.7 \\
Antenna\_Coupling & \faTable & 86.3 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gBad 0.0 & - & \gGood 88.8 & \gHigh 100.0 & \gHigh 91.3 & \gMid 55.7 & \gMid 67.2 & \gGood 79.2 & \gMid 70.8 & \gMid 70.0 & \gLow 49.7 & \gHigh 100.0 \\
Tokamak\_Dust\_Dynamics & \faTable & 85.1 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gMid 65.1 & \gMid 55.0 & - & \gHigh 100.0 & \gMid 70.0 & \gHigh 100.0 & \gGood 83.3 & \gLow 47.0 \\
Coherent\_Light\_Int. & \faTable & 85.0 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 80.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gMid 65.0 & - & - & \gGood 81.2 & \gMid 70.0 & \gGood 76.5 & \gMid 55.0 \\
SUSY & \faTable & 84.6 & \gMid 52.0 & \gBad 0.0 & \gGood 75.0 & \gBad 0.0 & \gHigh 98.9 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 99.7 & \gMid 72.9 & \gGood 89.0 & \gGood 85.0 & \gGood 82.5 & \gGood 88.1 \\
BOUT\_Impur.\_Migr. & \faGlobe & 82.4 & \gGood 80.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & - & - & - & \gGood 87.4 & \gBad 20.0 & - & - & \gGood 81.2 & \gHigh 100.0 & \gLow 49.6 & \gHigh 100.0 \\
Laser\_Chirp\_EUV & \faImage & 82.2 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gMid 66.7 & \gGood 86.7 & \gHigh 100.0 & \gMid 63.7 & \gMid 67.7 & \gMid 60.9 & \gGood 86.7 & - & \gHigh 100.0 & \gGood 80.0 & \gGood 82.9 & \gHigh 98.9 \\
Superheavy\_Nuclei & \faTable & 81.3 & \gGood 76.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 85.3 & \gHigh 90.6 & \gHigh 100.0 & \gHigh 100.0 & \gBad 0.0 & \gLow 44.8 & \gBad 0.0 & \gMid 56.9 & \gBad 0.0 & \gHigh 92.0 & \gLow 30.0 & \gHigh 95.0 \\

\rowcolor{green!8} \multicolumn{18}{c}{\textit{\textbf{Biology}}} \\
\midrule
Flysta3D & \faImage & 91.4 & - & - & - & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 99.6 & \gMid 71.2 & - & \gHigh 100.0 & \gHigh 98.1 & \gHigh 100.0 & \gMid 53.3 & - \\
The-Gonzo-Dataset & \faGlobe,\faTable & 86.8 & \gHigh 100.0 & \gMid 55.6 & \gGood 83.3 & \gHigh 100.0 & \gLow 48.8 & - & \gHigh 100.0 & \gHigh 100.0 & \gGood 78.3 & - & - & \gHigh 100.0 & \gHigh 100.0 & \gGood 82.7 & \gHigh 100.0 \\
Synth.-Skeletal-Mot. & \faImage,\faTable & 81.4 & \gHigh 100.0 & \gLow 44.4 & \gGood 83.3 & \gHigh 100.0 & \gMid 50.0 & \gHigh 96.8 & \gHigh 100.0 & \gGood 87.7 & \gMid 68.0 & \gGood 84.5 & \gHigh 91.0 & \gHigh 92.2 & \gMid 60.0 & \gGood 86.3 & \gGood 87.1 \\
MedMNISTv2 & \faGlobe & 80.2 & \gHigh 100.0 & \gMid 55.6 & \gGood 83.3 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 92.1 & \gHigh 100.0 & \gMid 70.0 & \gGood 75.6 & \gGood 80.3 & - & \gGood 85.0 & \gMid 74.7 & \gBad 6.0 & \gGood 85.2 \\
FIVES & \faImage & 80.0 & \gLow 36.0 & \gMid 55.6 & \gMid 58.3 & \gHigh 100.0 & \gBad 0.0 & \gHigh 97.6 & \gHigh 99.4 & \gHigh 90.0 & \gHigh 91.4 & \gHigh 99.8 & - & \gGood 87.5 & \gHigh 92.0 & \gMid 55.0 & \gHigh 96.5 \\
Genomic-benchmarks & \faFont & 79.9 & \gMid 60.0 & \gMid 66.7 & \gMid 66.7 & \gHigh 90.6 & \gGood 78.1 & \gMid 70.0 & \gHigh 100.0 & \gHigh 94.0 & \gGood 79.9 & \gHigh 98.6 & - & \gMid 62.5 & \gGood 80.0 & \gBad 0.0 & \gHigh 96.1 \\
RNA-seq-human-kidney & \faTable & 79.8 & \gMid 60.0 & \gMid 66.7 & \gMid 62.5 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 100.0 & \gHigh 95.3 & \gMid 64.1 & \gHigh 100.0 & \gBad 0.0 & \gMid 51.2 & \gHigh 100.0 & \gMid 50.7 & - \\
HQColon\_sampled & \faImage,\faGlobe,\faTable & 77.9 & \gMid 56.0 & \gMid 66.7 & \gMid 70.8 & \gBad 0.0 & \gGood 80.6 & \gBad 0.0 & \gGood 87.5 & \gHigh 98.0 & \gGood 81.1 & \gGood 80.4 & - & \gHigh 100.0 & \gHigh 100.0 & \gGood 76.7 & \gBad 16.7 \\
Insect-Odorant-Bind. & \faProjectDiagram,\faTable & 76.8 & \gHigh 96.0 & \gBad 22.2 & \gGood 79.2 & \gGood 87.5 & \gMid 63.5 & \gHigh 99.5 & \gHigh 94.7 & \gHigh 95.5 & \gMid 64.8 & \gHigh 93.7 & \gLow 25.7 & \gHigh 95.5 & \gGood 86.5 & \gGood 75.0 & \gGood 84.9 \\
RAS-Dataset & \faGlobe & 74.8 & \gHigh 96.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 75.0 & \gHigh 100.0 & \gHigh 100.0 & \gGood 78.0 & \gGood 86.9 & \gMid 62.5 & \gBad 5.9 & - & \gGood 77.1 & \gHigh 90.0 & \gBad 10.0 & \gMid 64.6 \\

\bottomrule
\end{tabular}
\end{table*}
